Assigning Medical Codes at the Encounter Level by Paying Attention to Documents

The vast majority of research in computer assisted medical coding focuses on coding at the document level, but a substantial proportion of medical coding in the real world involves coding at the level of clinical encounters, each of which is typically represented by a potentially large set of documents. We introduce encounter-level document attention networks, which use hierarchical attention to explicitly take the hierarchical structure of encounter documentation into account. Experimental evaluation demonstrates improvements in coding accuracy as well as facilitation of human reviewers in their ability to identify which documents within an encounter play a role in determining the encounter level codes.

==> ELDAN5.0 (2)/append_dataset.tex <==
\ignore{The experiment dataset includes 463,866 coded encounters containing 1,390,605 documents in the corpus, 31\% (145,518) of the encounters containing a single document. In the remaining 69\% of the dataset, encounter documentation contained an average of 3.91~documents; see }
Table~\ref{tbl:corpus} shows a histogram of encounters that contain a specific number of documents.

\begin{table}[h!]
\centering
\begin{adjustbox}{angle=90,width=0.4\columnwidth}
\begin{tabular}{r|rl}
% \rotatebox[origin=c]{270}{\#doc in encounter }  &  \rotatebox[origin=c]{270}{count}       &                \\
&  & \# of encounters \\ \midrule
& & \\
\rotatebox[origin=c]{270}{1}  &  145,518 &  \mybar{20.79} \\
\rotatebox[origin=c]{270}{2}  &  113,706 &  \mybar{16.24} \\
\rotatebox[origin=c]{270}{3}  &   72,580 &  \mybar{10.37} \\
\rotatebox[origin=c]{270}{4}  &   45,864 &   \mybar{6.55} \\
\rotatebox[origin=c]{270}{5}  &   28,364 &   \mybar{4.05} \\
\rotatebox[origin=c]{270}{6}  &   17,935 &   \mybar{2.56} \\
\rotatebox[origin=c]{270}{7}  &   12,242 &   \mybar{1.75} \\
\rotatebox[origin=c]{270}{8}  &    8,274 &   \mybar{1.18} \\
\rotatebox[origin=c]{270}{9}  &    5,648 &   \mybar{0.81} \\
\rotatebox[origin=c]{270}{10} &    3,989 &   \mybar{0.57} \\
\rotatebox[origin=c]{270}{11} &    2,863 &   \mybar{0.41} \\
\rotatebox[origin=c]{270}{12} &    2,190 &   \mybar{0.31} \\
\rotatebox[origin=c]{270}{13} &    1,663 &   \mybar{0.24} \\
\rotatebox[origin=c]{270}{14} &    1,217 &   \mybar{0.17} \\
\rotatebox[origin=c]{270}{15} &     997 &   \mybar{0.14} \\
\rotatebox[origin=c]{270}{16} &     816 &   \mybar{0.12} \\
\end{tabular}
\end{adjustbox}


\# of documents in an encounter
\caption{Histogram of the number of documents in an encounter. %\# of encounter is the number of encounters that contains the respective number of documents. 
\label{tbl:corpus}}
\vspace{-1em}
\end{table}

==> ELDAN5.0 (2)/append_doc_f1.tex <==
\label{ap:doc_f1}

\begin{table}[h!]

\centering
\caption{An illustration of how ELDAN's document attention predictions are evaluated using source documents labeled by human coders. Green (the shading under Human Coders) indicates the ``source'' documents for the encounter-level code (truth), and gray (the shading under Eldan's Document Attention) indicates the documents with high attention (prediction). The bolded documents are the true positives. In this example, the precision is $\frac{tp}{tp + fp}=\frac{3}{3 + 2} = \frac{3}{5}$. The recall is $\frac{tp}{tp + fn}=\frac{3}{3 + 1} = \frac{3}{4}$. The document-level F1 score is thus $\frac{2}{3}$.}
\resizebox{0.50\columnwidth}{!}{%
\begin{tabular}{r|r|r}
\toprule
Encounter & ELDAN's Document Attention & Human Coders\\
\midrule
$enc_1$ & $[\mathcolorbox{lightgray}{\bf{doc_1}}, \mathcolorbox{lightgray}{doc_2}, doc_3]$ & $[\mathcolorbox{green}{\bf{doc_1}}, doc_2, doc_3]$ \\
\midrule
$enc_2$ & $[\mathcolorbox{lightgray}{\bf{doc_4}}]$ & $[\mathcolorbox{green}{\bf{doc_4}}]$ \\
\midrule
$enc_3$ & $[doc_5, \mathcolorbox{lightgray}{\bf{doc_6}}, doc_7, \mathcolorbox{lightgray}{doc_8}]$ & $[\mathcolorbox{green}{doc_5}, \mathcolorbox{green}{\bf{doc_6}}, doc_7, doc_8]$ \\
\bottomrule
\end{tabular}
}

\label{tb:atten-example}
\end{table}

\ignore{In addition to reporting the document-level F1-score, we report, for each code, the number of encounters that contain the code, the number of documents in those encounters, and the number of ``source'' documents labeled by medical coders. Finally,}
To calculate document-level F1-score, we limit our encounters to those that contain the targeted code based on the encounter-level labels, since~(1) there are no annotations for documents that are not in those encounters, and~(2) for ELDAN, attention on the negative encounter can imply negative correlation, which is irrelevant to what we want to evaluate.


==> ELDAN5.0 (2)/append_model.tex <==
\label{ap:model}

The overall architecture of Encounter-Level Document Attention Networks (ELDAN) is shown in Figure~\ref{fig:eldan}. It 
%is an extension of Hierarchical Attention Networks~\citep{yang2016hierarchical} and 
consists of three parts: (1)~a document-level encoder that turns sparse document features into dense document features, (2)~a document-level attention layer\ignore{ that draws inspiration from~\citet{yang2016hierarchical}}, and (3)~an encounter-level encoder. 
%We first introduce notation and then describe the three parts in more details.

\begin{figure}[h!]
  \centering 
  \includegraphics[width=0.7\textwidth]{ELDAN.pdf} 
  \caption{Architecture of Encounter-Level Document Attention Network (ELDAN)}
  \label{fig:eldan}
\end{figure} 


\ignore{As multiple codes are often associated with an encounter, encounter-level coding can be considered a multi-label classification problem. \hancomment{Added justification for our decision to train one-vs-all binary}
%For simplicity, 
For our interest in evaluating the interpretability of ELDAN, we decompose the problem into multiple one-vs-all binary classification problems, with each one targeting one code $c_t \in C = \{c_1, c_2, \cdots, c_K\}$, the set of all codes. This adds flexibility in potential use cases where specific codes of interest could vary across sites or even dynamically, and it makes it easier to compare code-specific document attention learned from the model to document annotations labeled by medical coders.\footnote{We do plan to explore ELDAN with multi-label classification in future work.} }
\psrcomment{Guoli should confirm the ``flexibility in potential use cases'' observation is true and ok to include, or feel free to delete it, keeping just the ``makes it easier to compare...'' piece.}

Let the set of encounters be $E = \{e_1, e_2, \cdots, e_n\}$, and their corresponding labels be $Y = \{y_1, y_2, \cdots, y_n\}$, where $y_i \in \{-1, 1\}$ represents whether the encounter $e_i$ contains the targeted medical code $c_t$. Each encounter $e_i$ comprises multiple documents, and the number of documents that an encounter contains can vary across encounters. Finally, let $x_{i,j}$ and $d_{i,j}$ be the sparse and dense feature vectors that represent document $j$ in encounter $i$, respectively.

\paragraph{Document-Level Encoder.}
\label{sec:d-encode}

The goal of the document-level encoder is to transform a sparse document representation, $x_{i,j}$, into a dense document representation, $d_{i,j}$. The sparse document representation, $x_{i,j}$ is first passed into an embedding layer, to map the 775,330-dimensional sparse document representation into a 300-dimensional vector. It is then followed by two fully-connected layers to produce a dense document representation, $d_{i,j}$.

\vspace{-1em}

\begin{align}
    h_{i,j,0} &= W_{Embedding} x_{i,j} \label{eq:embedding}\\ 
    h_{i,j,1} &= tanh \left ( W_{FC_1} h_{i,j,0} + b_{FC_1} \right ) \\
    d_{i,j} &= tanh \left ( W_{FC_2} h_{i,j,1} + b_{FC_2} \right )
\end{align}

\vspace{-0.5em}

\noindent where $W$ represents the weight matrix, $b$ represents a bias vector, and tanh is the hyperbolic tangent. $h_{i,j,0}$ and $h_{i,j,1}$ are hidden representations of document $j$ in encounter $i$.

\paragraph{Document-Level Attention.}
\label{sec:d-atten}

\ignore{When a medical code is assigned to an encounter, it does not imply that all the documents in the encounter contain evidence for the medical code. If we directly aggregate (whether by summing or averaging) all the dense document representations in that encounter, $\{d_{i,1}, d_{i,2}, \cdots, d_{i,m}\}$, we will typically end up including irrelevant information that dilutes the signal of the presence of medical code. Instead, we might want a weighted average, where the more relevant documents are being paid more attention. }To calculate attention for a document, the dense document representation $d_{i,j}$ is compared to a learnable attention vector, $v_{attention}$, after passing through a fully-connected layer and a non-linear layer. Specifically,

\vspace{-1em}

\begin{align}
        u_{i,j} &= tanh\left ( W_{FC_3} d_{i,j} + b_{FC_3} \right ) \label{eq:transformation_ap}  \\
        a_{i,j} &= \frac{exp\left (u_{i,j}^\top v_{attention}\right )}{\sum_{j=1}^m exp\left (u_{i,j}^\top v_{attention}\right )} \label{eq:atten_ap} \\
        e_{i} &= \sum_{j=1}^m a_{i,j} d_{i,j} \label{eq:avg_ap}
\end{align}

\vspace{-1em}

\noindent where $a_{i,j}$ is the normalized attention score for document $j$ in encounter $i$, and $e_{i}$ is the encounter representation of encounter $i$. As shown in Equation~\ref{eq:atten_ap}, the transformed document representation $u_{i,j}$ is compared with the learnable attention vector $v$ using dot product, and further normalized for the weighted averaging step in Equation~\ref{eq:avg_ap}.

\paragraph{Encounter-Level Encoder.}
\label{sec:e-encode}

Once we have the encounter representation $e_i$, we can predict whether the encounter contains the targeted medical code. Specifically,

\vspace{-1em}

\begin{equation}
    P(\hat{y_i}) = softmax\left ( W_{FC_4} e_{i} + b_{FC_4} \right )
\end{equation}

\vspace{-0.5em}

\noindent Finally, we compare with the ground truth label of encounter $i$ using negative log-likelihood to calculate a loss 
$- log \left ( p(\hat{y_i} = y_i) \right )$ on encounter $i$, where $y_i$ is the ground-truth label. 

\ignore{
\vspace{-1em}
\begin{equation}
\label{eq:loss}
    Loss_i = - log \left ( p(\hat{y_i} = y_i) \right )
\end{equation}
\vspace{-0.7em}
\noindent where $y_i$ is the ground-truth label. 
}

\label{sec:model_training}
\paragraph{Training details.}
Our 80-10-10 dataset split results in 371,092 encounters for training, 46,387 encounters for development/tuning, and 46,387 encounters for testing. Note that no document-level annotations are available. We train models implemented with PyTorch~\citep{paszke2017automatic} on the~150 most frequent codes, using minibatch stochastic gradient descent~\citep{Sutskever:2013:IIM:3042817.3043064} with a minibatch size of 64, learning rate of 0.01, and a momentum of 0.9. Since we are in an imbalanced setting (some medical codes can be extremely rare, see Fig.~\ref{tb:average}), we randomly resampled the training data by assigning different probability to the positive and negative classes so that the ratio of positive encounters and negative encounters is close to $1:6$. No resampling is done for the development set and test set. These hyperparameters were selected based on our results on the development set.

For na\"ive transfer learning, models are trained from the most frequent code to the least frequent. The model for the most frequent code is trained from scratch just like \textsc{ELDAN}. For all the other models, the weight of the $(n)$-th most frequent model's embedding layer ($W_{Embedding}$, see Equation~\ref{eq:embedding}) is first initialized (but not fixed) by that of the $(n-1)$-th most frequent model prior to training.

==> ELDAN5.0 (2)/append_results.tex <==

THIS APPENDIX SECTION HAS BEEN RE-INTEGRATED WITH THE MAIN BODY OF THE PAPER

\ignore{
As shown in Table~\ref{tb:top20_svm}, \textsc{ELDAN} consistently outperforms the baseline \ignore{\textsc{ELDN}, the version of \textsc{ELDAN} without attention,} for 17 out of the most frequent 20 codes. This demonstrates the effectiveness of an attention mechanism on the document level. \ignore{This makes sense, as during the medical coding process, some documents can be more important compared to other documents for making a decision on whether to code the specific medical code.} 


% comparing ELDAN to ELDAN+transfer
%\psrcomment{The first three sentences here belong in results.tex and the start of this paragraph should be a briefer reminder about what ELDAN+transfer is, if that's even needed.}


% comparing ELDAN to Logistic Regression
% \hancomment{Comparing ELDAN to Logistic Regression, waiting for the training to finish (at least of the top 20 codes). One important note: right now, only 16 models are trained (in 2 days), and I need 150. I don't think I can finish the experiment before Friday... Do you think it would hurt us very much if we only use ELDN as our baseline? I suspect that for the top 20 codes ELDAN is better than Logistic Regression, but for the rest Logistic Regression will actually be better, because it has smaller amount of parameters to train.}

\begin{table}[h!]
\centering
\caption{Encounter-level F1-scores of 20 most frequent CPT codes. \#Docs is the average number of documents found in the encounters that contain the code. Prevalence is the percentage of all encounters that contain that code.}
\resizebox{0.55\columnwidth}{!}{%
\begin{tabular}{l|rr|r|rr}
\toprule
{CPT Codes} &  \#Docs & Prevalence & \textsc{ELDN} &    \textsc{ELDAN} & \thead{\textsc{ELDAN}\\\textsc{+transfer}}  \\
\midrule
43239   &       3.13 &     4.15\% &       84.59 &  \bf{86.21} &          84.93 \\
45380   &       2.78 &     3.56\% &       72.68 &  \bf{75.14} &          74.02 \\
45385   &       2.75 &     2.44\% &       71.33 &  \bf{72.33} &          70.31 \\
66984   &       2.51 &     1.90\% &       92.15 &       92.87 &     \bf{93.00} \\
45378   &       2.40 &     1.89\% &       62.67 &       65.45 &     \bf{67.57} \\
12001   &       2.20 &     1.60\% &  \bf{46.96} &       44.74 &          43.62 \\
12011   &       2.35 &     1.19\% &       41.03 &       42.12 &     \bf{43.30} \\
29125   &       2.85 &     1.05\% &       52.32 &  \bf{56.50} &          54.10 \\
10060   &       2.09 &     1.00\% &       45.15 &       48.73 &     \bf{52.25} \\
69436   &       3.01 &     0.96\% &       83.30 &       85.18 &     \bf{88.32} \\
12002   &       2.60 &     0.92\% &       25.53 &       28.36 &     \bf{28.43} \\
59025   &       1.86 &     0.92\% &  \bf{73.82} &       69.00 &          67.73 \\
11042   &       3.20 &     0.88\% &       64.38 &       63.45 &     \bf{66.86} \\
47562   &       4.36 &     0.80\% &       70.74 &       76.25 &     \bf{77.67} \\
62323   &       2.10 &     0.79\% &       61.17 &       57.07 &     \bf{64.25} \\
\midrule
\midrule
Average &       2.62 &            &       58.02 &       60.40 &     \bf{61.26} \\     
\bottomrule
\end{tabular}
}

\label{tb:top20_svm}
\vspace{-0.5em}
\end{table}
}

==> ELDAN5.0 (2)/conclusion.tex <==

In this paper, we have introduced a new approach to encounter-level coding that explicitly takes the hierarchical structure of encounter documentation into account.
%, by extending hierarchical attention networks~\citep{yang2016hierarchical}
Experimental validation of the model shows that it improves coding accuracy against a strong baseline, and also supports the conclusion that its assignment of document-level attention would provide value in helping human coders to identify document-level evidence for encounter-level codes during review. We also found that, in a setting using a set of one-vs-all classifiers, a na\"ive transfer learning approach was surprisingly effective in helping to deal with rare codes.

\ignore{
    \item Implementation-level innovations needed to scale ELDAN up to a real-world number of codes. \hancomment{I am not so sure about this being a strong contribution now, as all other deep learning people just train one multi-label model, instead of 50 binary models, which help with the speed.}
    \item Naive transfer learning \hancomment{(reference to Hal’s work and follow-ons) I read through Hal's work, I think it is probably a stretch to make a connection?}: which is surprising effective for helping with rare codes.
}



==> ELDAN5.0 (2)/dataset.tex <==

\hancomment{This section is for Guoli to write, but here are some info that would be very nice if it can make it in: 

(1) the corpus is outpatient data (as inpatient data does not have CPT code), 

(2) how the feature extraction is being done, like using UMLS or rule-based approach to identify concept etc..., and possibly mentioning that we have 775330 features?
}

We used outpatient procedure (CPT) coding production data internal to 3M Health Information Systems, a leading provider of CAC solutions, sampled from multiple hospital sites.
Our dataset includes 463,866 coded encounters containing 1,390,605 documents, with 31\% of encounters containing a single document; in the remainder, there are an average of 3.91~documents per encounter.
We generated a random 80-10-10 training/tuning/evaluation split by encounter ID. Coding exists only at the encounter level, with no indication of which codes are associated with which document(s).\footnote{To eliminate risk of inappropriate protected health information (PHI) transmission even internally within 3M HIS, once documents were selected, they were immediately converted from their original form to feature vectors containing UMLS CUIs (Concept Unique Identifiers) and 3M HIS
%3M HIS 
internal numeric concept identifiers as well as words or phrases  (775,330 unique features) for all downstream machine learning development and experimentation. 
%3M HIS
No PHI contributed to the features used to represent documents.}
\ignore{; see Table~\ref{tbl:corpus} for finer-grained details.}
\hancomment{added according to Guoli's reply}
\ignore{Outpatient encounters typically include multiple documents, }
\ignore{ history and physical exams, progress reports, discharge summaries, consultations, as well as lab and radiology reports. \ignore{although there are no guarantee that all of these will be available.}}



\ignore{
\subsection{Feature Choices} 
To eliminate PHI (Patient Health Information) exposure, all the data used in this experiment are derived data from original EHR (Electronic Health Record). The derived data is in the format of "feature vector" for each document, and the features in the feature vector are NLP contents, which could be No PHI is used as feature. 
}


%Because it's prohibitively expensive to use SMEs (Subject-matter Experts) to do large scale annotation to associate encounter level human codes to the document(s) belongs to the encounter, a 3M HIS proprietary NLP tool was used to automatically associate encounter level codes to the underlined documents for all the encounters in the corpus based on "retrospective evidence" technique. 

%"Retrospective evidence" technique basically takes a (putatively correct) code, and identify where in the document it could have been generated. One example of doing this is to use the official description of the code, or other language variations associated with it, and match in the document. For example, ICD-10 code S72.301A can be described as “initial encounter for closed fracture of the shaft of the right femur”.  If S72.301A is an encounter-level code, the technique could be used to look for documents containing supporting text, e.g. finding “Patient came in immediately following an auto collision …  Right femur fracture,  closed.”

In addition, to assess the value of document-level attention in identifying which documents are responsible for encounter codes (for facilitating human code review) we extracted a separate dataset from production data, comprising 393 encounters.\footnote{To eliminate possible leakage across experiments these do not overlap with the first set.} \psrcomment{Can we verify that none of the \emph{patients} overlap? Ideally in the train/dev/test split above also? This is a much stronger statement than just saying the encounters do not overlap}For each encounter, experienced medical coders annotated \emph{document}-level codes corresponding to the encounter-level coding. Specifically, coders were instructed to read through all the documents contained in the encounter, and assign a code from the encounter level to the document if (and only if) it contains sufficient evidence for assigning the code. Note this means the same code can be assigned to multiple documents within the encounter. 



==> ELDAN5.0 (2)/discussion.tex <==

\paragraph{Results Evaluating Encounter-Level Code Prediction.} 
\textsc{ELDAN} consistently outperforms the baseline\ignore{\textsc{ELDN}, the version of \textsc{ELDAN} without attention,} for 17 of the most frequent 20 codes (Fig.~\ref{tb:top20_svm}, left).
To show the trend across the full range of codes we macro-average every 10 codes from most frequent to least frequent (Fig.~\ref{tb:top20_svm}, right). \textsc{ELDAN} with or without na\"ive transfer learning consistently outperforms \textsc{ELDN}, even for extremely rare codes ($<0.1\%$). As codes become rarer, \textsc{ELDAN+transfer} tends toward outperforming \textsc{ELDAN} more substantially; see increasing trend for $\Delta$\textsc{ELDAN}. This improvement can be explained by viewing the embedding layer as a vector space model that maps sparse features that are extracted from the document (such as medical concepts, UMLS CUIs) to a dense representation, which can be effective for bootstrapping the training of rare codes.

\begin{figure}[ht]
\centering
\caption{\underline{\emph{Left}}: Encounter-level F1-scores of the 20 most frequent CPT codes.\ \#Docs is the average number of documents found in the encounters that contain the code; prevalence is the percentage of all encounters that contain that code. \underline{\emph{Right}}: Macro average of encounter-level F1 scores for every 10 codes (from most to least frequent). $\Delta$\textsc{ELDAN} $=  \textsc{ELDAN+transfer}  - \textsc{ELDAN}$.
\label{tb:top20_svm} \label{tb:average}
}
\vspace{0.5em}
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{l|rr|r|rr}
\toprule
{CPT Codes} &  \#Docs & Prevalence & \textsc{ELDN} &    \textsc{ELDAN} & \thead{\textsc{ELDAN}\\\textsc{+transfer}}  \\
\midrule
43239   &       3.13 &     4.15\% &       84.59 &  \bf{86.21} &          84.93 \\
45380   &       2.78 &     3.56\% &       72.68 &  \bf{75.14} &          74.02 \\
45385   &       2.75 &     2.44\% &       71.33 &  \bf{72.33} &          70.31 \\
66984   &       2.51 &     1.90\% &       92.15 &       92.87 &     \bf{93.00} \\
45378   &       2.40 &     1.89\% &       62.67 &       65.45 &     \bf{67.57} \\
12001   &       2.20 &     1.60\% &  \bf{46.96} &       44.74 &          43.62 \\
12011   &       2.35 &     1.19\% &       41.03 &       42.12 &     \bf{43.30} \\
29125   &       2.85 &     1.05\% &       52.32 &  \bf{56.50} &          54.10 \\
10060   &       2.09 &     1.00\% &       45.15 &       48.73 &     \bf{52.25} \\
69436   &       3.01 &     0.96\% &       83.30 &       85.18 &     \bf{88.32} \\
12002   &       2.60 &     0.92\% &       25.53 &       28.36 &     \bf{28.43} \\
59025   &       1.86 &     0.92\% &  \bf{73.82} &       69.00 &          67.73 \\
11042   &       3.20 &     0.88\% &       64.38 &       63.45 &     \bf{66.86} \\
47562   &       4.36 &     0.80\% &       70.74 &       76.25 &     \bf{77.67} \\
62323   &       2.10 &     0.79\% &       61.17 &       57.07 &     \bf{64.25} \\
\midrule
\midrule
Average &       2.62 &            &       58.02 &       60.40 &     \bf{61.26} \\     
\bottomrule
\end{tabular}
\ \ \ \ \ \ 
\begin{tabular}{r|r|r|rr|r}
\toprule
{Average} & Prevalence &   \textsc{ELDN} &       \textsc{ELDAN} & \thead{\textsc{ELDAN}\\\textsc{+transfer}} & $\Delta$\textsc{ELDAN} \\
\midrule
1st to 10th    &     1.97\% &  65.22 &       66.93 &     \bf{67.14} &   0.22 \\
11st to 20th   &     0.78\% &  50.82 &       53.87 &     \bf{55.38} &   1.50 \\
21st to 30th   &     0.51\% &  55.93 &  \bf{63.07} &          62.23 &  -0.85 \\
31st to 40th   &     0.40\% &  44.93 &       51.92 &     \bf{55.24} &   3.32 \\
41st to 50th   &     0.30\% &  32.08 &       38.61 &     \bf{39.35} &   0.74 \\
51st to 60th   &     0.26\% &  33.83 &       38.80 &     \bf{39.10} &   0.30 \\
61st to 70th   &     0.23\% &  28.37 &       35.05 &     \bf{36.62} &   1.56 \\
71st to 80th   &     0.21\% &  25.66 &       30.62 &     \bf{32.93} &   2.31 \\
81st to 90th   &     0.18\% &  34.92 &       42.03 &     \bf{43.26} &   1.23 \\
91st to 100th  &     0.16\% &  24.54 &       29.06 &     \bf{31.32} &   2.25 \\
101st to 110th &     0.14\% &  25.15 &       33.17 &     \bf{34.57} &   1.40 \\
111st to 120th &     0.12\% &  24.87 &       31.74 &     \bf{32.84} &   1.09 \\
121st to 130th &     0.11\% &  18.14 &       24.10 &     \bf{28.09} &   3.99 \\
131st to 140th &     0.10\% &  20.39 &       28.53 &     \bf{32.21} &   3.68 \\
141st to 150th &     0.08\% &  26.93 &       33.13 &     \bf{40.94} &   7.82 \\
\bottomrule
\end{tabular}
}
\vspace{-0.2em}
\end{figure}




\begin{table}[ht]
\centering
\caption{Document-level F1-score calculated by comparing document attention from \textsc{ELDAN} and human coders on 20 CPT codes. \#enc is the number of encounters that contains the code. \#doc is the number of documents within those encounters. \#source is the number of documents being labeled by human coders as the source documents for the code.
%\#enc miss is the number of encounters within the original annotation that human coders did not found any evidence for the code. 
Attention (from \textsc{ELDAN}) and Chance both report document-level F1-score, and Diff is the difference between them.}

\resizebox{1.0\columnwidth}{!}{%

\resizebox{0.40\columnwidth}{!}{%
\begin{tabular}{l|rrr|rr|r}
\toprule
{CPT Codes} &  \#enc &  \#doc&  \#source &  Attention &  Chance &  Diff \\
\midrule
43239 &               8 &                       19 &              9 &      88.89 &   59.22 & 29.67 \\
45380 &               5 &                       11 &              5 &      90.91 &   56.47 & 34.44 \\
45385 &               6 &                       13 &              8 &      85.71 &   67.52 & 18.20 \\
66984 &               7 &                       13 &              7 &     100.00 &   68.65 & 31.35 \\
45378 &              10 &                       20 &             11 &      90.91 &   67.44 & 23.47 \\
12001 &               1 &                        3 &              1 &     100.00 &   45.63 & 54.37 \\
12011 &               3 &                        8 &              3 &      57.14 &   54.30 &  2.85 \\
29125 &               2 &                        9 &              4 &      72.73 &   50.91 & 21.81 \\
10060 &               4 &                        9 &              6 &     100.00 &   71.65 & 28.35 \\
69436 &               7 &                       18 &              8 &      87.50 &   60.54 & 26.96 \\
\bottomrule
\end{tabular}
}

\hspace{0.5em}

\resizebox{0.40\columnwidth}{!}{%
\begin{tabular}{l|rrr|rr|r}
\toprule
{CPT Codes} &  \#enc &  \#doc&  \#source &  Attention &  Chance &  Diff \\
\midrule
12002 &               4 &                       13 &              6 &      92.31 &   56.02 & 36.29 \\
59025 &             0 &                      0 &            0 &        - &     - &   - \\
11042 &               5 &                       23 &             16 &      58.06 &   64.89 & -6.82 \\
47562 &               1 &                        5 &              3 &     100.00 &   57.62 & 42.38 \\
62323 &               5 &                       11 &              7 &      87.50 &   69.85 & 17.65 \\
64483 &               3 &                        8 &              4 &     100.00 &   58.07 & 41.93 \\
43235 &               6 &                       18 &              6 &      83.33 &   45.19 & 38.15 \\
20610 &               5 &                        9 &              5 &     100.00 &   72.25 & 27.75 \\
49083 &              10 &                       27 &             13 &      85.71 &   60.21 & 25.50 \\
51702 &               2 &                        2 &              2 &     100.00 &  100.00 &  0.00 \\
\bottomrule
\end{tabular}
}
}

\label{tb:attention}

\vspace{-0.2em}

\end{table}


%On document attention compared with human
%\psrcomment{I actually think you might want separate subsections, one for the classification, and one for this result.}
\paragraph{Results Evaluating Relevant-Document Prediction against Human Judgments.}
Table~\ref{tb:attention} shows document-level F1-score for the most frequent~20 encounter-level codes, with surprisingly strong results: 100\% F1-score on 7 out of 19 available codes.\footnote{Note that as the dataset is smaller and disjoint from the training dataset, codes can be missing (such as code 59025).} However, even chance performance could be good if the number of possible documents to assign credit to is very small.\footnote{As an extreme case, performance for code 51072 is evaluated on two encounters, each of which contains only a single document (Table~\ref{tb:attention}), though this is atypical.} Therefore we compare
to the chance baseline. ELDAN is consistently better, usually by a large margin.\footnote{Except for one code. Improvement is significant at p < .05 using a one-sample t-test comparing the population mean of average F1 over the 500 chance baseline runs against the document-level F1 obtained using the document attention model.} These results support the conclusion that ELDAN's document attention is effective in identifying signal from ``source'' documents for the targeted code --- crucially, without training on document-level annotations.


\ignore{
 number of documents in those encounters that contain the code, as well as the number of ``source'' documents labeled by human coders in Table~\ref{tb:attention}. It is evident that for many high performing codes, the strong results hold.
}
 \ignore{For the one code that it does worse, the difference is relatively low, and could be due to variance resulted from evaluating on a small dataset.} 
%For the only two codes in the top 20 most frequent codes that \textsc{ELDAN} does not outperform \textsc{ELDAN}, code \textsc{12001} is simple repair of superficial wounds of scalp, neck, axillae, external genitalia, trunk and/or extremities (including hands and feet) that is less then 2.5 cm, and code \textsc{59025} is a fetal non-stress test (FNST), the monitoring of the fetal heart rate in response to fetal movement. As our dataset is an outpatient dataset (meaning that the patient did not stay over at the hospital), these two codes could imply that


==> ELDAN5.0 (2)/experiments.tex <==

\ignore{Our first validation experiment tests ELDAN's effectiveness for predicting encounter-level codes. The second looks at the value of document-level attention from ELDAN as a prediction of which documents in the encounter can be considered the ``source'' for the encounter-level codes.}

\ignore{
We first talk about how the training is set up and the implementation innovation \hancomment{might be too strong, as I used many existing pytorch modules.} needed to scale ELDAN to 150 codes, and then talk about the experiment designs.
}


\paragraph{Evaluating Encounter-Level Code Prediction.}
%\label{sec:enc_per}
% commented out to save space
% \paragraph{Implementation.}
% Our model is implemented with PyTorch~\citep{paszke2017automatic}. As training~150 neural models posed a computational challenge, we optimized the design of our network in several ways. First, as the number of documents in an encounter can vary (from~1 to~16 in our case), na\"ively batching the encounter can lead to unnecessary overhead. We utilize the \textsc{PackedSequence} data structure in PyTorch to collect all the documents in a minibatch of encounters, and concurrently pass all the documents through the document encoder layer. The documents, after being converted to a dense representation, are then redistributed back to the respective encounters with the correct ordering before passing into the document attention layer. For the document encoder layer, we have also experimented with using bidirectional gated recurrent units (GRU) on the document level, but found little to no difference on the performance, and thus use a fully-connected network instead for extra speedup. Finally, as our inputs are sparse document features (775,330 dimensional, with each document typically consisting of about 5,000 non-zero features), multiplying that by any matrix can be time consuming. We therefore utilize an \textsc{EmbeddingBag} layer to handle the sparse matrix multiplication. These design choices, taken together, reduced our training time for one model from around 1,800 minutes to around 150 minutes.\ignore{\footnote{Trained on a 64GB RAM machine with 16 CPU. No GPU was used, due to privacy concern for transferring data to another machine.}} \psrcomment{I have removed the footnote about GPUs because it contradicts the earlier comment about representing documents as CUIs and concept IDs to make sure they contain no PHI during experimentation.  If we did that, why would GPUs be a privacy concern?}
We train two \textsc{ELDAN} models. One is a standard \textsc{ELDAN} model (Section~\ref{sec:model} and Appendix~\ref{sec:model_training}). The other, which we refer to as \textsc{ELDAN+transfer}, includes a simple but effective enhancement for handling rare codes, since, when the code is rare, training a deep one-vs-all network can be challenging. To address this issue, we use a na\"ive transfer learning technique that initializes the embedding layer \ignore{($W_{Embedding}$)}with that of a trained model on a more frequent code.\footnote{See Appendix~\ref{sec:model_training}, under Training Details. We call this na\"ive as it is clearly not optimal nor novel, but the results demonstrate a potentially promising direction for training classifiers for rare medical codes in settings where a single multi-label classifier may be less desirable for other reasons, as discussed above.}
%See Table~\ref{tb:top20_svm} and Table~\ref{tb:average} for the results.
We measure performance in standard fashion using the F1 score.

We regard Yang et al.'s \citep{yang2016hierarchical} non-attention hierarchical network (HN-AVE in their paper) as a strong baseline since,
in experiments across six document classification datasets, they demonstrated that it substantially outperformed a range of typical baselines lacking hierarchy; these included, for example, bag of words, SVM, LSTM, and CNN classifiers. \suggestignore{(They then demonstrated consistent further improvement for hierarchical network modeling with attention.) }Analogously, we define \textsc{ELDN} (encounter level document network) as a baseline that simply averages documents rather than using attention.\footnote{Note that most prior methods for medical coding base the prediction on a single discharge summary (which is rarely present in outpatient encounters), and are thus not applicable as baselines in our setting.} \suggestignore{Specifically, an equally weighted average is used to combine dense document representations, $\{d_{i,1}, d_{i,2}, \cdots, d_{i,m}\}$, into an encounter representation, $e_i$. } 


%presumed to be an upper bound on non-neural or non-hierarchical neural methods.

% \textbf{\textsc{Logistic Regression}}:
% \hancomment{As we might not be able to report the production-level SVM (and the comparison may be unfair), I coded up a logistic regression that is currently running. One important note: right now, only 16 models are trained (in 2 days), and I need 150. I don't think I can finish the experiment before Friday... Do you think it would hurt us very much if we only use ELDN as our baseline?} A standard logistic regression trained on the encounter level, following the same resampling technique used to train the ELDAN model. To get the encounter feature, we use the same sparse document features used in ELDAN, and average them to get a encounter-level feature.

% \textbf{\textsc{SVM}}:
% A document-level one vs. all support vector machine (SVM). The SVM is trained on the document level, using the label of its encounter as the document label. The prediction results of the documents are then merged into a encounter prediction by taking the union of the documents in the encounter. Note that this result is obtained from a different but similar dataset, therefore not directly comparable. We include it as a reference.

%\vspace{-0.5em}
\paragraph{Evaluating Relevant-Document Prediction against Human Judgments.} To evaluate the extent to which document attention learned by \textsc{ELDAN} matches human medical coders' judgments about the documents relevant for coding the encounter, we apply our trained models to our second dataset. Recall that this is a separate set of 393~encounters for which a team of experienced medical coders annotated codes at the document level.
%The medical coders were instructed to read through all the documents contained in the encounters, and assign the code to the document if the document contains sufficient evidence for assigning the code. This means that the code can be assigned to multiple documents within the encounter.
We calculate \textit{document-level F1-score} by treating document attention learned from \textsc{ELDAN} as the prediction of which documents are the ``source'', and comparing this to medical coders' ground truth --- see Appendix~\ref{ap:doc_f1} for an illustration. Note that this is different from the encounter-level F1 scores used to evaluate encounter-level code prediction.
%Table~\ref{tb:attention} shows the document-level f1-score for the same 20 codes as reported in Table~\ref{tb:top20_svm}. 

To determine which \emph{documents} are predicted to contain targeted codes (therefore relevant for human code review of the encounter-level coding), we pass the annotated dataset through the \textsc{ELDAN} model trained for encounter-level code prediction, with no further tuning or training. We then use a selection strategy that takes the attention scores of all the documents in an encounter\ignore{(which can be viewed as a multinomial distribution),} and marks all documents that are strictly larger then half the maximum attention score as containing the targeted code. \suggestignore{Note we did not tune this heuristic strategy on the evaluation dataset: the $0.5$ threshold was determined by the observation on the development set that attention scores are often skewed, but sometimes there exist two or more documents with similar high scores.}Since a baseline to compare with document-level attention can be non-trivial to implement, in the spirit of having a chance-adjusted measure, we compare with a baseline obtained by randomly generating attention scores from a uniform distribution on the documents within an encounter, then following the same selection strategy as in ELDAN's document attention selection. The chance baseline is run~500 times to reduce the noise level.


==> ELDAN5.0 (2)/future.tex <==

% Combining solution (1) and (2). Use an encounter level model, but use (1) as weak supervision for the document attention assignment.

In future work, we are particularly interested in exploring the further potential afforded by the assignment to individual documents of credit for encounter-level codes. ELDAN's document-attention can be viewed as a multinomial distribution across documents in an encounter, weighting candidate source documents.  This can be interpreted as a form of weak supervision, and incorporated either via the loss function, or by bringing human judgments back into the loop, e.g. applying active learning to focus on obtaining high quality annotations for valuable subsets of noisily-annotated documents.
An additional focus for future work will be to explore ELDAN with multi-task and multi-label learning, as well as further variants of na\"ive transfer, taking advantage of domain knowledge by grouping codes from the same code family together.


==> ELDAN5.0 (2)/introduction.tex <==

\textit{Medical coding} translates unstructured information about diagnoses, treatments, procedures, medications and equipment into alphanumeric codes\ignore{, such as International Classification of Diseases (ICD) codes or Current Procedural Terminology (CPT) codes,} for billing\ignore{or insurance} purposes.
\ignore{To correctly interpret this information, experienced professionals (known as medical coders)}Coding is challenging and expensive, requiring high-expertise professionals,\ignore{Experienced medical coders  involved in the process of medical coding. However, this can be expensive due to the large amount of medical text that needs to be processed, a high degree of expertise is required,}
and even experienced coders frequently disagree with each other \citep{resnik2006using}.
Increasingly, computer assisted coding (CAC) is used to help address these issues by automatically suggesting medical codes, generally within a workflow that supports subsequent human review to ensure that codes are correct or to make revisions.

\ignore{
Significant progress has been made on accurate code assignment and on presenting results in a way that coders can interpret (e.g.~\citep{Mullenbach2018ExplainablePO, baumel2018multi}), and auto-suggestion has been shown to improve inter-coder consistency~\citep{resnik2006using}.
}

The vast majority of relevant literature focuses on automatic code assignment at the document level, such as radiology reports \citep[e.g.][]{farkas2008automatic} or discharge summaries \citep[e.g.][]{perotte2013diagnosis}. However, in many settings codes are assigned not to individual documents, but to an entire medical \emph{encounter},\ignore{i.e. an interaction between a patient and healthcare provider,} such as a patient visit to a hospital.
%\hancomment{should we emphasis here that in certain encounter, such as out-patient, discharge summary is not available, thus using discharge summary as proxy to encounter has inherent limitations?}
%\footnote{An encounter is defined as ``(1) an instance of direct provider/practitioner to patient interaction, regardless of the setting, between a patient and a practitioner vested with primary responsibility for diagnosing, evaluating or treating the patients condition, or both, or providing social worker services; (2) A contact between a patient and a practitioner who has primary responsibility for assessing and treating the patient at a given contact, exercising independent judgment.'' (ASTM E1384-02a -- Standard Guide for Content and Structure of the Electronic Health Record)} 
Encounter-level documentation often involves multiple documents~\citep{o2005measuring},
%\ignore{, such as history and physical, operative reports, radiology reports, physician's orders, \ignore{progress and nursing notes, consultations, discharge summary,} etc.\ignore{, based on the encounter setting~}}
%The outpatient encounters are generally much shorter than inpatient encounters, since there is no overnight stay in outpatient. In inpatient setting the number of documents in an encounter depends on severity of a patient illness and the length of stay~\citep{o2005measuring}.
%The documentation for clinical encounters can comprise multiple documents ranging from a simple diagnosis report by a clinician, to a paper trail that could include, for example, admission diagnoses, radiology reports, progress and nursing notes, and discharge summary, spanning over the duration of days or weeks~\citep{o2005measuring}.
%\hancomment{not sure if the above example is correct, check with coders to make sure}\psrcomment{I agree: important to check}
%\ignore{and assigning codes to sets of documents, rather than individual documents,creates additional challenges, for computer assisted coding, }
and the relationship between the encounter-level codes and the unstructured information in the documents is indirect --- so the standard approach, treating coding as a well understood kind of text classification problem~\citep[e.g.][]{Pang:2002:TUS:1118693.1118704, Wang:2012:BBS:2390665.2390688,yang2016hierarchical}, does not map naturally to document \textit{collections}.
% In this paper, we present the Encounter-Level Document Attention Network (ELDAN) to jointly address these criteria. The ELDAN is a recurrent neural network that uses an attention mechanism to highlight pertinent documents and phrases for the coder to pay attention to, and it assigns codes at the encounter level.
% \subsection{Goal}
% Accurately assist humans in assigning medical codes to a medical encounter while also providing explainability.
% This goal can be broken down into sub-goals: 
% \begin{enumerate}
%     \item Accurately: 
%         high accuracy (f1) on code prediction
%     \item assist humans: 
%     result has to be interpretable, with human-in-the-loop (why the code is predicted, from which documents)
%     human has to be able to identify the source of the error to improve the system.
%     \item assigning medical codes to a medical encounter
%     the assignment is on the encounter level. 
%     each encounter could have multiple codes, each code could manifest in a subset of the documents in the encounter.
%     For simplicity, we do not consider a structured lab value associated with that encounter.
% \end{enumerate}
% \subsection{Technical Challenges}
% \ignore{
% One approach to address this problem is to 
% %distribute encounter-level codes into document-level and 
% train a \textit{document-level} model and then, at prediction time, merge predicted document codes into encounter codes. This approach has the benefit of reducing the problem to document classification, which is well-studied. The challenge, however, is that when a medical coder assigns a medical code, it is on the medical encounter level, 
% %So coded training data contain codes at the encounter level, and i
% and it is unclear how to distribute the encounter-level codes down to the document-level in order to obtain document-level training data. The presence of a code in an encounter certainly does not imply that \emph{all} the documents in the encounter have evidence for that code, and information on specifically which documents are the ``source'' of the encounter-level code is usually not provided in the coding process. Merging document-level codes is also not a trivial task: as pointed out by~\citet{o2005measuring}, a more specific code may suppress more general codes, complicating the process.
% %A possible solution to this problem, which we will discuss further in Section~\ref{}, is a knowledge-based evidence filter: if you cannot find any evidence of a medical code in a document, then that document probably does not contain the medical code.
% }
One obvious solution, using document-level models and then merging their predictions into encounter codes, immediately runs up against a lack of training data: medical coders do not identify which documents are the ``source'' for each encounter code. In addition, merging document-level codes involves non-trivial interactions, e.g. specific codes suppressing more general codes~\citep{o2005measuring}. 

In this paper, we instead focus on training an \textit{encounter-level} model directly.
%\ignore{This has the benefit of not needing to worry about how document-level codes relate to the encounter level.}
One straightforward approach would be to aggregate (via sum or average) all document features into a single encounter feature set, but this would be noisy, as the signal of the targeted medical code is diluted when irrelevant documents are also included. It also fails to address the crucial problem of \emph{interpretability}: human coders reviewing auto-suggested codes need to relate proposed encounter codes back to document-level evidence.\footnote{Interpretability is also important from a technical perspective, to identify problems in the prediction model.}
% \hancomment{talk about why interpretablility is important for coder to make decision, and why interpretablility is important for debugging?}
We therefore introduce a new approach to encounter-level coding, observing that its structure is essentially hierarchical, progressing from textual evidence up to documents, and from there to entire encounters\ignore{ where the labels are to be found}. Our Encounter-Level Document Attention Network (ELDAN) applies the key insights of hierarchical attention networks~\citep[HAN,][]{yang2016hierarchical},
% \ignore{and as such it
% operates hierarchically at multiple levels, both the encounter and document level, using attention. Attention }
enabling the model to
%\ignore{derive an appropriate focus on which}
%textual evidence is most relevant to documents, and then which 
identify which documents are most relevant in encounters as driven by the encounter-level task.  
We obtain positive results for encounter-level labeling in comparison to a strong, realistic baseline, and also show that the resulting weighting helps coders identify which documents are likely sources for a code.

\ignore{ --- this permits investigation of specific documents, either to review suggested encounter codes or to identify problems in the prediction model.}


%\hancomment{talks about how CPT codes (focusing on procedure) are different from ICD codes, and it is less studied in the literature of automatic clinical coding?}

% We know how to classify a document. However, the ground-truth assignment is based on the encounter level (which is a collection of documents). Saying an encounter has code `A’ doesn’t mean all the documents has code `A’. This convolutes the problem of code assignment and interpretability, specifically

% How to predict code on encounter-level?
% Which subset of the documents are the ``source’’ of the medical code?

% Another problem related to medical code prediction:

% ->>>>>>>>>> move to other place?
% Finally, another challenge for medical code prediction is that the medical codes can be severely imbalanced, CPT (Current Procedural Terminology) codes for example, common ones are around 8\%, rare ones can be around 0.0\%. In the cases of rare medical codes, data sparsity can also be an issue for training complex model.

% \subsection{Solutions}

% Two possible solutions:

% \begin{enumerate}
%     \item Distribute encounter-level codes into document-level, train a document-level model. At prediction time, merge the predicted document codes into encounter codes.
%     \begin{enumerate}
%         \item Pro: We know how to train a document-level model.
%         \item Challenge: Distribute encounter-level code into document-level can be difficult.
%         \item Solution: Knowledge-based evidence filter: if you can’t find any evidence of a code in a document, then that document probably doesn\'t contain the code.
%     \end{enumerate}

%     \item Train an encounter-level model.
    
%     \begin{enumerate}
%         \item Pro: Do not need to worry about distributing codes and merging them afterward.
%         \item Challenge: How to train an encounter-level model? Can the model be interpretable such that we know which subset of the documents are the ``source'' of the medical code?
%         \item Solution: Hierarchical Attention Model (HAN): Attention enables the model to have the ability to assign different weights to different document when combining them. Attention also allows interpretation, in that it enables a human to understand which documents are likely candidate for the codes. This allows human to investigate specific document to identify the problem. 
%     \end{enumerate}
    




% \end{enumerate}


% \subsection{Data Imbalance and Sparsity}

% Imbalance: downsample the negative class to somewhere between POS:NEG = 1:6.

% \noindent Sparsity: Naive transfer learning, use the embedding layer of the previously trained model as the starting point. (help with performance on low resource codes)



% make sure that the core ideas can be understood by
% an informed reader in either community.  And certainly this
% introduction should be readable by all!  In fact, every introduction
% should have the following two sections:

% \paragraph{Technical Significance}
% Give us a few sentences about what methods you extend.  You'll have a
% more detailed related work, but for now you should tell us what is
% your key technical contribution.  Make sure you follow up with details
% in the methods section and appendices.  \emph{Lack of technical
%   details, such that the methods can be verified, is a major reason
%   that otherwise strong-looking papers are scored low/rejected.}

% \paragraph{Clinical Relevance}
% Give us a few sentences about how your work is going to improve
% healthcare.  MLHC is not interested in another DNN on another clinical
% data set; this part must convince a clinician that your work matters.
% \emph{Unclear clinical contributions are a major reason that otherwise
%   strong-looking papers are scored low/rejected.}

\ignore{
Our main contributions with this paper are:

\begin{enumerate}
    \item The extension of hierarchical attention network~\citep{yang2016hierarchical} (HAN) to encounter-level coding.
    \item Evaluation not only of code quality, but of accuracy when identifying evidence for reviewers.
    \item Implementation-level innovations needed to scale ELDAN up to a real-world number of codes. \hancomment{I am not so sure about this being a strong contribution now, as all other deep learning people just train one multi-label model, instead of 50 binary models, which help with the speed.}
    \item Naive transfer learning \hancomment{(reference to Hal’s work and follow-ons) I read through Hal's work, I think it is probably a stretch to make a connection?}: which is surprising effective for helping with rare codes.
\end{enumerate}
}



==> ELDAN5.0 (2)/model.tex <==
The overall architecture of Encounter-Level Document Attention Networks (ELDAN)
%is an extension of Hierarchical Attention Networks~\citep{yang2016hierarchical} and 
consists of three parts: (1)~a document-level encoder that turns sparse document features into dense document features using an embedding layer followed by two fully connected layers, (2)~a document-level attention layer that draws inspiration from~\citet{yang2016hierarchical}, and (3)~an encounter-level encoder using a fully connected layer. See Appendix~\ref{ap:model} for full description.
%We first introduce notation and then describe the three parts in more details.

\ignore{As multiple codes are often associated with an encounter,} Encounter-level coding can be considered a multi-label classification problem. \hancomment{Added justification for our decision to train one-vs-all binary}
%For simplicity, 
We decompose the problem into multiple one-vs-all binary classification problems, each targeting one code\ignore{$c_t \in C$, the set of all codes}, which adds flexibility for use cases where codes of interest could vary across sites or even dynamically, and also facilitates comparing code-specific document attention learned from the model to document annotations labeled by medical coders, in our evaluation below.\footnote{We also plan to explore ELDAN with multi-label classification in future work.} 
\psrcomment{Guoli should confirm the ``flexibility in potential use cases'' observation is true and ok to include, or feel free to delete it, keeping just the ``makes it easier to compare...'' piece.}

\ignore{
Let $(E,Y)$ be $n$ encounters with corresponding labels, where each $y_i \in \{-1, 1\}$ represents whether encounter $e_i$ contains the targeted medical code $c_t$. Each encounter $e_i$ comprises multiple documents, and the number of documents in an encounter can vary. Finally, let $x_{i,j}$ and $d_{i,j}$ be the sparse and dense feature vectors that represent document $j$ in encounter $i$, respectively.
}
\ignore{
\paragraph{Document-Level Encoder.}
\label{sec:d-encode}

The goal of the document-level encoder is to transform a sparse document representation, $x_{i,j}$, into a dense document representation, $d_{i,j}$. The sparse document representation, $x_{i,j}$ is first passed into an embedding layer, to map the 775,330-dimensional sparse document representation into a 300-dimensional vector. It is then followed by two fully-connected layers to produce a dense document representation, $d_{i,j}$.

\vspace{-1em}

\begin{align}
    h_{i,j,0} &= W_{Embedding} x_{i,j} \\ 
    h_{i,j,1} &= tanh \left ( W_{FC_1} h_{i,j,0} + b_{FC_1} \right ) \\
    d_{i,j} &= tanh \left ( W_{FC_2} h_{i,j,1} + b_{FC_2} \right )
\end{align}

\vspace{-0.5em}

\noindent where $W$ represents the weight matrix, $b$ represents a bias vector, and tanh is the hyperbolic tangent. $h_{i,j,0}$ and $h_{i,j,1}$ are hidden representations of document $j$ in encounter $i$.
}

\ignore{
\paragraph{Document-Level Attention.}
\label{sec:d-atten}
} 

When a code is assigned to an encounter, it does not imply that all its documents contain evidence for that code. Directly summing or averaging all the encounter's dense document representations \ignore{in that encounter, $\{d_{i,1}, d_{i,2}, \cdots, d_{i,m}\}$, we} will typically capture irrelevant information, diluting the signal for the presence of the code. Instead, ELDAN computes a weighted average, where more relevant documents receive more attention. This is calculated by comparing the dense document representation to a learnable attention vector, after passing through a fully connected-layer and a non-linear layer (see Appendix~\ref{ap:model}, especially eqs. \ref{eq:transformation_ap}-\ref{eq:avg_ap}).

\ignore{
\vspace{-1em}

\begin{small}
\begin{align}
        u_{i,j} &= tanh\left ( W_{FC_3} d_{i,j} + b_{FC_3} \right ) \\
        a_{i,j} &= \frac{exp\left (u_{i,j}^\top v_{attention}\right )}{\sum_{j=1}^m exp\left (u_{i,j}^\top v_{attention}\right )} \label{eq:atten} \\
        e_{i} &= \sum_{j=1}^m a_{i,j} d_{i,j} \label{eq:avg}
\end{align}
\end{small}

\vspace{-1em}

\noindent where $a_{i,j}$ is the normalized attention score for document $j$ in encounter $i$, and $e_{i}$ is the encounter representation of encounter $i$. \ignore{As shown in Equation~\ref{eq:atten}, the transformed document representation $u_{i,j}$ is compared with the learnable attention vector $v$ using dot product, and further normalized for the weighted averaging step in Equation~\ref{eq:avg}.}
}

\ignore{
\paragraph{Encounter-Level Encoder.}
\label{sec:e-encode}

Once we have the encounter representation $e_i$, we can predict whether the encounter contains the targeted medical code. Specifically,

\vspace{-1em}

\begin{equation}
    P(\hat{y_i}) = softmax\left ( W_{FC_4} e_{i} + b_{FC_4} \right )
\end{equation}

\vspace{-0.5em}

\noindent Finally, we compare with the ground truth label of encounter $i$ using negative log-likelihood to calculate a loss 
$- log \left ( p(\hat{y_i} = y_i) \right )$ on encounter $i$, where $y_i$ is the ground-truth label. 

\ignore{
\vspace{-1em}
\begin{equation}
\label{eq:loss}
    Loss_i = - log \left ( p(\hat{y_i} = y_i) \right )
\end{equation}
\vspace{-0.7em}
\noindent where $y_i$ is the ground-truth label. 
}
}

% \section{Implementation Innovation for Scalability}

% \hancomment{talk about implementation details, such as EmbeddingBag, PackPadSequence? (mainly about speedup) Maybe a dedicated section?}

% \begin{align}
%         u_{i} &= tanh\left ( W_e _{i} + b_e \right ) \\
%         a_{i,j} &= \frac{u_{i,j}^\top v}{\sum_{j=1}^m u_{i,j}^\top v} \label{eq:atten} \\
%         e_{i} &= \sum_{j=1}^M a_{i,j} d_{i,j} \label{eq:avg}
% \end{align}



% \begin{enumerate}
%     \item For each document in the encounter
%     \begin{enumerate}
%         \item A feature extractor is used to extract a document-level sparse feature for each document.
%         \item Each document-level sparse feature is passed through an embedding layer to convert into a document-level dense feature.
%         \item Each document-level dense feature is then passed through two fully connected hidden layers to convert into the final document level feature.
%         \item An attention vector is multiplied with the document level feature of each documents in the encounter. The results is normalized to weights (i.e. attentions). 
%         \item These weights (attentions) are then used to weighted average the document-level features into a single encounter level feature.
%     \end{enumerate}
    
%     \item The encounter level feature is then passed through another fully connected layer and a softmax layer, to produce a score that represents the negative log likelihood of the encounter having the targeted medical code. 
% \end{enumerate}


==> ELDAN5.0 (2)/related.tex <==

\ignore{
The automatic identification of medical codes dates back at least to~1973, when~\citet{dinwoodie1973automatic} proposed a dictionary matching method based on clinical code descriptions. Since the 1990s, a growing literature has introduced natural language processing techniques to address the task of automatic clinical coding using the unstructured text data~\citep[][ and many others]{resnik2006using,Pestian2007AST,Zhang2017EnhancingAI,Mullenbach2018ExplainablePO}. Many of these studies, however, focus on limited categories of codes, such as variations of pneumonia, or only analyze specific subsets of clinical documents, such as chest radiology and discharge summary~\citep{stanfill2010systematic}. Progress on this problem using state of the art techniques has also been hampered significantly by the broader research community's limited access to large, shareable datasets~\citep{resnikDataRant2018}.
}
% version 1
% % version 2
% More recently, due to the advancement of deep learning, many neural models have been applied to automatic clinical coding,
\ignore{
More recently, particularly thanks to the availability of a large public dataset, MIMIC III~\citep{johnson2016mimic}, machine learning work on medical coding has moved toward a more comprehensive approach to the problem.  At the same time, 
%the literature tends to focus on ICD coding, in contrast to our focus on CPT~codes, and 
}
Most work in CAC is limited to discharge summaries~\citep[e.g.][]{perotte2013diagnosis,stanfill2010systematic}, which are assumed to condense information about a patient stay. This can be problematic: \citet{kripalani2007deficits}\ignore{reviewing~73 published studies investigating hospital communication and information transfer}  find high rates of information missing from discharge summaries,\ignore{including median missing-information rates of 10.5\% for physical findings, 38\% for diagnostic test results, and,} notably 17.5\% missing the main diagnosis.\ignore{, which would therefore need to be identified from other documentation in the encounter.}
%we have found that on the order of 20\% of codes still need to be identified from other documentation in the encounter. 
In addition, for outpatient encounters discharge summaries are rarely a part of the record.\footnote{\ignore{An expert medical coder observes that this makes sense, since for}The patient is generally not admitted to the facility, and thus will not be discharged.}

Deep learning models have been applied to CAC, \ignore{viewing it as part of an assisted coding process and}some exploiting attention mechanisms to support explainability \citep{baumel2018multi,Mullenbach2018ExplainablePO,shi2017towards}. Crucially, however, these all look solely at the discharge summary. To our knowledge, our work is the first to investigate the hierarchical structure of the encounter as a whole.
% \ignore{
% \citet{baumel2018multi} extend hierarchical attention networks to a multi-label setting, and~\citet{shi2017towards} use hierarchical attention in a character-level LSTM model looking at both the discharge summary and clinical code descriptions. \citet{Mullenbach2018ExplainablePO} also aim to improve the explanability of the model by introducing a convolutional neural network with attention that aims to highlight segments of words in the discharge summary that lead to the prediction.
% }
% \ignore{
% Attention mechanisms in deep learning allow the network to focus on specific ``regions'' of the input data, which has proven helpful in, among others, machine translation~\citep{bahdanau2014neural}, summarization~\citep{rush2017neural}, and sentiment analysis~\citep{yang2016hierarchical}. Attention, especially in the context of NLP, has two main advantages: it allows the network to attend to meaningful parts of the sequence (either words or sentences), often leading to improved performance, and it provides insight into which parts of the sequence are being used to make the prediction.\footnote{Though see recent discussion
% in \citet{Jain2019AttentionIN,wiegreffe2019attention,wallace2019response}.}  These characteristics have made attention mechanisms a popular choice for deep learning in automatic clinical coding~\citep{baumel2018multi, shi2017towards, Mullenbach2018ExplainablePO}. 
% }
Our work draws inspiration from \citet{yang2016hierarchical}, who use a hierarchical word-to-sentence-to-document architecture in sentiment analysis.\ignore{They use a two-level attention mechanism that learns to pay attention to specific words in a sentence to form a sentence representation, and at the next higher level to weight specific sentences in a document in forming a document representation.}~Our own multi-level architecture 
progresses from sparse document features to dense document vectors to encounters.\ignore{work moves a level up the representational hierarchy, learning also to weight documents to form encounter representations. Instead of building the representation from the word level, our work}
Domain-informed feature extraction using 
subject matter knowledge and resources, e.g. UMLS,
\ignore{allows us to incorporate expert knowledge, helps alleviate the problem of out-of-vocabulary and uncommon abbreviation terms often found in clinical notes, and}
permits a shallower network, therefore requiring less training data, which is important in a setting where many codes are rare.

% \begin{enumerate}
%     \item Medical coding in general 
%     \item Encounter-level coding
%     \item Human in the loop, especially with regard to understanding why codes were assigned
%     \item Hierarchical attention networks
% \end{enumerate}


==> ELDAN5.0 (2)/results.tex <==




% 43239   &       3.13 &     4.15\% &  \bf{86.21} &          84.93 &       84.59 \\
% 45380   &       2.78 &     3.56\% &  \bf{75.14} &          74.02 &       72.68 \\
% 45385   &       2.75 &     2.44\% &  \bf{72.33} &          70.31 &       71.33 \\
% 66984   &       2.51 &     1.90\% &       92.87 &     \bf{93.00} &       92.15 \\
% 45378   &       2.40 &     1.89\% &       65.45 &     \bf{67.57} &       62.67 \\
% 12001   &       2.20 &     1.60\% &       44.74 &          43.62 &  \bf{46.96} \\
% 12011   &       2.35 &     1.19\% &       42.12 &     \bf{43.30} &       41.03 \\
% 29125   &       2.85 &     1.05\% &  \bf{56.50} &          54.10 &       52.32 \\
% 10060   &       2.09 &     1.00\% &       48.73 &     \bf{52.25} &       45.15 \\
% 69436   &       3.01 &     0.96\% &       85.18 &     \bf{88.32} &       83.30 \\
% 12002   &       2.60 &     0.92\% &       28.36 &     \bf{28.43} &       25.53 \\
% 59025   &       1.86 &     0.92\% &       69.00 &          67.73 &  \bf{73.82} \\
% 11042   &       3.20 &     0.88\% &       63.45 &     \bf{66.86} &       64.38 \\
% 47562   &       4.36 &     0.80\% &       76.25 &     \bf{77.67} &       70.74 \\
% 62323   &       2.10 &     0.79\% &       57.07 &     \bf{64.25} &       61.17 \\
% 64483   &       2.10 &     0.77\% &  \bf{67.32} &          66.74 &       54.27 \\
% 43235   &       2.91 &     0.75\% &  \bf{38.77} &          35.45 &       31.43 \\
% 20610   &       2.11 &     0.75\% &       46.75 &     \bf{48.60} &       43.90 \\
% 49083   &       2.33 &     0.62\% &       71.49 &     \bf{75.08} &       58.24 \\
% 51702   &       2.78 &     0.59\% &       20.30 &          22.96 &  \bf{24.74} \\
% \midrule
% \midrule
% Average &            &            &       60.40 &     \bf{61.26} &       58.02 \\

% \begin{table}[]
% \centering
% \begin{tabular}{l|ll|lll|l}
% \toprule
% {CPT Codes} &  \#doc per enc & percentage &       ELDAN & ELDAN+transfer &        ELDN &         SVM \\
% \midrule
% 43239   &       3.13 &     5.18\% &  \bf{86.21} &          84.93 &       84.59 &       80.59 \\
% 45380   &       2.78 &     4.45\% &  \bf{75.14} &          74.02 &       72.68 &       66.37 \\
% 45385   &       2.75 &     3.06\% &  \bf{72.33} &          70.31 &       71.33 &       69.81 \\
% 66984   &       2.51 &     2.37\% &       92.87 &     \bf{93.00} &       92.15 &       79.62 \\
% 45378   &       2.40 &     2.36\% &       65.45 &     \bf{67.57} &       62.67 &       62.91 \\
% 12001   &       2.20 &     2.01\% &       44.74 &          43.62 &  \bf{46.96} &       30.37 \\
% 12011   &       2.35 &     1.49\% &       42.12 &     \bf{43.30} &       41.03 &       37.75 \\
% 29125   &       2.85 &     1.32\% &  \bf{56.50} &          54.10 &       52.32 &       10.54 \\
% 10060   &       2.09 &     1.24\% &       48.73 &     \bf{52.25} &       45.15 &       23.79 \\
% 69436   &       3.01 &     1.20\% &       85.18 &          88.32 &       83.30 &  \bf{92.42} \\
% 12002   &       2.60 &     1.14\% &       28.36 &     \bf{28.43} &       25.53 &       21.36 \\
% 59025   &       1.86 &     1.14\% &       69.00 &          67.73 &  \bf{73.82} &        3.20 \\
% 11042   &       3.20 &     1.10\% &       63.45 &     \bf{66.86} &       64.38 &       42.64 \\
% 47562   &       4.36 &     1.00\% &       76.25 &          77.67 &       70.74 &  \bf{85.72} \\
% 62323   &       2.10 &     0.99\% &       57.07 &     \bf{64.25} &       61.17 &       33.58 \\
% 64483   &       2.10 &     0.96\% &       67.32 &          66.74 &       54.27 &  \bf{72.64} \\
% 43235   &       2.91 &     0.94\% &  \bf{38.77} &          35.45 &       31.43 &       25.07 \\
% 20610   &       2.11 &     0.94\% &       46.75 &          48.60 &       43.90 &  \bf{60.66} \\
% 49083   &       2.33 &     0.78\% &       71.49 &     \bf{75.08} &       58.24 &       37.71 \\
% 51702   &       2.78 &     0.74\% &       20.30 &          22.96 &  \bf{24.74} &        8.40 \\
% \midrule
% \midrule
% Average &            &            &       60.40 &     \bf{61.26} &       58.02 &       47.26 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT codes}
% \label{tb:top20_svm}
% \end{table}



% \begin{table}[]
% \centering
% \begin{tabular}{lllll}
% \toprule
% {CPT Code} & percentage &       ELDAN & ELDAN+transfer &        ELDN \\
% \midrule
% 43239         &     4.15\% &  \bf{86.21} &          84.93 &       84.59 \\
% 45380         &     3.56\% &  \bf{75.14} &          74.02 &       72.68 \\
% 45385         &     2.43\% &  \bf{72.33} &          70.31 &       71.33 \\
% 66984         &     1.90\% &       92.87 &     \bf{93.00} &       92.15 \\
% 45378         &     1.89\% &       65.45 &     \bf{67.57} &       62.67 \\
% 12001         &     1.60\% &       44.74 &          43.62 &  \bf{46.96} \\
% 12011         &     1.20\% &       42.12 &     \bf{43.30} &       41.03 \\
% 29125         &     1.04\% &  \bf{56.50} &          54.10 &       52.32 \\
% 10060         &     1.00\% &       48.73 &     \bf{52.25} &       45.15 \\
% 69436         &     0.96\% &       85.18 &     \bf{88.32} &       83.30 \\
% 12002         &     0.91\% &       28.36 &     \bf{28.43} &       25.53 \\
% 59025         &     0.91\% &       69.00 &          67.73 &  \bf{73.82} \\
% 11042         &     0.89\% &       63.45 &     \bf{66.86} &       64.38 \\
% 47562         &     0.80\% &       76.25 &     \bf{77.67} &       70.74 \\
% 62323         &     0.79\% &       57.07 &     \bf{64.25} &       61.17 \\
% 64483         &     0.77\% &  \bf{67.32} &          66.74 &       54.27 \\
% 20610         &     0.75\% &       46.75 &     \bf{48.60} &       43.90 \\
% 43235         &     0.75\% &  \bf{38.77} &          35.45 &       31.43 \\
% 49083         &     0.63\% &       71.49 &     \bf{75.08} &       58.24 \\
% 51702         &     0.58\% &       20.30 &          22.96 &  \bf{24.74} \\
% \midrule
% \midrule
% Average &            &       60.40 &     \bf{61.26} &       58.02 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT codes\hancomment{Logistic Regression to be added later}}
% \label{tb:top20_svm}
% \end{table}



% \begin{table}[]
% \centering
% \begin{tabular}{llll}
% \toprule
% {} &       ELDAN & ELDAN+transfer &        ELDN \\
% \midrule
% 43239         &  \bf{86.21} &          84.93 &       84.59 \\
% 45380         &  \bf{75.14} &          74.02 &       72.68 \\
% 45385         &  \bf{72.33} &          70.31 &       71.33 \\
% 66984         &       92.87 &     \bf{93.00} &       92.15 \\
% 45378         &       65.45 &     \bf{67.57} &       62.67 \\
% 12001         &       44.74 &          43.62 &  \bf{46.96} \\
% 47562         &       76.25 &     \bf{77.67} &       70.74 \\
% 44970         &  \bf{70.63} &          69.63 &       63.97 \\
% 29125         &  \bf{56.50} &          54.10 &       52.32 \\
% 69436         &       85.18 &     \bf{88.32} &       83.30 \\
% 11042         &       63.45 &     \bf{66.86} &       64.38 \\
% 12011         &       42.12 &     \bf{43.30} &       41.03 \\
% 12002         &       28.36 &     \bf{28.43} &       25.53 \\
% 43235         &  \bf{38.77} &          35.45 &       31.43 \\
% 52332         &  \bf{47.38} &          44.63 &       36.90 \\
% 10060         &       48.73 &     \bf{52.25} &       45.15 \\
% 58558         &       58.88 &     \bf{60.27} &       52.12 \\
% 52356         &  \bf{63.61} &          58.48 &       47.79 \\
% 27447         &       52.20 &     \bf{59.35} &       47.72 \\
% 59025         &       69.00 &          67.73 &  \bf{73.82} \\
% \midrule
% \midrule
% Macro Average &       61.89 &     \bf{62.00} &       58.33 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT code (without SVM)}
% \label{tb:top20}
% \end{table}









% \begin{enumerate}
%     \item Check with Guoli about the details of the experiment data for code assignment.
        
%         Need to make sure there is a reasonable story about this being a valid comparison (even if the datasets in the experimental conditions were only comparable, not identical, because of the need to compare against a highly tuned, production-level system).
        
%         Also need to check with Guoli about it being ok to report numbers from the production-level system.
        
%     \item Performance comparison:
%     \begin{enumerate}
%         \item Models:
%         \begin{enumerate}
%             \item ELDAN
%             \item ELDN (without attention, just averaging)
%             \item SVM OVA (3M current model, solution (1))
%         \end{enumerate}
        
%         \item ELDAN consistently outperforms ELDN with about 1.5 f1-score
%         \item Compared with SVM OVA, ELDAN outperform on common codes, but not as competitive when codes are rare (although in most cases, both models don\'t work well.)
%         \item Low resource codes: The effect of naive transfer learning (a consistent improvement of 1 f1-score, especially for rare codes) 
%     \end{enumerate}
    
%     \item Attention:
    
%     Experienced medical coder hand-labeled 400 encounters. 
% High f1 of document source assignment compared to human using ELDAN.
    
% \end{enumerate}


% \subsection{Evaluation Approach/Study Design} 

% Before jumping into the results: what exactly are you evaluating?
% Tell us (or remind us) about your study design and evaluation
% criteria.  

% \subsection{Results on Application A} 

% Give us some numbers about how well your awesomeness works, especially
% in comparison to some baselines.  You should provide a summary of the
% results in the text, as well as in tables (such as
% table~\ref{tab:example}) and figures (such as figure~\ref{fig:example}).  

% You may use subfigures/wrapfigures so that figures don't have to span
% the whole page or multiple figures are side by side.

% \begin{table}[htbp]
%   \centering 
%   \caption{These are our results.} 
%   \begin{tabular}{|l|l|}\hline
%     Us & Top Score \\ \hline
%     Baseline & Less Impressive Score \\ \hline 
%   \end{tabular}
%   \label{tab:example} 
% \end{table}

% \begin{figure}[htbp]
%   \centering 
%   \includegraphics[width=1.5in]{smile.jpeg} 
%   \caption{Feeling awesome.}
%   \label{fig:example} 
% \end{figure} 

% \subsection{Results on Application B} 

% Did more than one experiment type?  Sweet! 

==> results.tex <==




% 43239   &       3.13 &     4.15\% &  \bf{86.21} &          84.93 &       84.59 \\
% 45380   &       2.78 &     3.56\% &  \bf{75.14} &          74.02 &       72.68 \\
% 45385   &       2.75 &     2.44\% &  \bf{72.33} &          70.31 &       71.33 \\
% 66984   &       2.51 &     1.90\% &       92.87 &     \bf{93.00} &       92.15 \\
% 45378   &       2.40 &     1.89\% &       65.45 &     \bf{67.57} &       62.67 \\
% 12001   &       2.20 &     1.60\% &       44.74 &          43.62 &  \bf{46.96} \\
% 12011   &       2.35 &     1.19\% &       42.12 &     \bf{43.30} &       41.03 \\
% 29125   &       2.85 &     1.05\% &  \bf{56.50} &          54.10 &       52.32 \\
% 10060   &       2.09 &     1.00\% &       48.73 &     \bf{52.25} &       45.15 \\
% 69436   &       3.01 &     0.96\% &       85.18 &     \bf{88.32} &       83.30 \\
% 12002   &       2.60 &     0.92\% &       28.36 &     \bf{28.43} &       25.53 \\
% 59025   &       1.86 &     0.92\% &       69.00 &          67.73 &  \bf{73.82} \\
% 11042   &       3.20 &     0.88\% &       63.45 &     \bf{66.86} &       64.38 \\
% 47562   &       4.36 &     0.80\% &       76.25 &     \bf{77.67} &       70.74 \\
% 62323   &       2.10 &     0.79\% &       57.07 &     \bf{64.25} &       61.17 \\
% 64483   &       2.10 &     0.77\% &  \bf{67.32} &          66.74 &       54.27 \\
% 43235   &       2.91 &     0.75\% &  \bf{38.77} &          35.45 &       31.43 \\
% 20610   &       2.11 &     0.75\% &       46.75 &     \bf{48.60} &       43.90 \\
% 49083   &       2.33 &     0.62\% &       71.49 &     \bf{75.08} &       58.24 \\
% 51702   &       2.78 &     0.59\% &       20.30 &          22.96 &  \bf{24.74} \\
% \midrule
% \midrule
% Average &            &            &       60.40 &     \bf{61.26} &       58.02 \\

% \begin{table}[]
% \centering
% \begin{tabular}{l|ll|lll|l}
% \toprule
% {CPT Codes} &  \#doc per enc & percentage &       ELDAN & ELDAN+transfer &        ELDN &         SVM \\
% \midrule
% 43239   &       3.13 &     5.18\% &  \bf{86.21} &          84.93 &       84.59 &       80.59 \\
% 45380   &       2.78 &     4.45\% &  \bf{75.14} &          74.02 &       72.68 &       66.37 \\
% 45385   &       2.75 &     3.06\% &  \bf{72.33} &          70.31 &       71.33 &       69.81 \\
% 66984   &       2.51 &     2.37\% &       92.87 &     \bf{93.00} &       92.15 &       79.62 \\
% 45378   &       2.40 &     2.36\% &       65.45 &     \bf{67.57} &       62.67 &       62.91 \\
% 12001   &       2.20 &     2.01\% &       44.74 &          43.62 &  \bf{46.96} &       30.37 \\
% 12011   &       2.35 &     1.49\% &       42.12 &     \bf{43.30} &       41.03 &       37.75 \\
% 29125   &       2.85 &     1.32\% &  \bf{56.50} &          54.10 &       52.32 &       10.54 \\
% 10060   &       2.09 &     1.24\% &       48.73 &     \bf{52.25} &       45.15 &       23.79 \\
% 69436   &       3.01 &     1.20\% &       85.18 &          88.32 &       83.30 &  \bf{92.42} \\
% 12002   &       2.60 &     1.14\% &       28.36 &     \bf{28.43} &       25.53 &       21.36 \\
% 59025   &       1.86 &     1.14\% &       69.00 &          67.73 &  \bf{73.82} &        3.20 \\
% 11042   &       3.20 &     1.10\% &       63.45 &     \bf{66.86} &       64.38 &       42.64 \\
% 47562   &       4.36 &     1.00\% &       76.25 &          77.67 &       70.74 &  \bf{85.72} \\
% 62323   &       2.10 &     0.99\% &       57.07 &     \bf{64.25} &       61.17 &       33.58 \\
% 64483   &       2.10 &     0.96\% &       67.32 &          66.74 &       54.27 &  \bf{72.64} \\
% 43235   &       2.91 &     0.94\% &  \bf{38.77} &          35.45 &       31.43 &       25.07 \\
% 20610   &       2.11 &     0.94\% &       46.75 &          48.60 &       43.90 &  \bf{60.66} \\
% 49083   &       2.33 &     0.78\% &       71.49 &     \bf{75.08} &       58.24 &       37.71 \\
% 51702   &       2.78 &     0.74\% &       20.30 &          22.96 &  \bf{24.74} &        8.40 \\
% \midrule
% \midrule
% Average &            &            &       60.40 &     \bf{61.26} &       58.02 &       47.26 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT codes}
% \label{tb:top20_svm}
% \end{table}



% \begin{table}[]
% \centering
% \begin{tabular}{lllll}
% \toprule
% {CPT Code} & percentage &       ELDAN & ELDAN+transfer &        ELDN \\
% \midrule
% 43239         &     4.15\% &  \bf{86.21} &          84.93 &       84.59 \\
% 45380         &     3.56\% &  \bf{75.14} &          74.02 &       72.68 \\
% 45385         &     2.43\% &  \bf{72.33} &          70.31 &       71.33 \\
% 66984         &     1.90\% &       92.87 &     \bf{93.00} &       92.15 \\
% 45378         &     1.89\% &       65.45 &     \bf{67.57} &       62.67 \\
% 12001         &     1.60\% &       44.74 &          43.62 &  \bf{46.96} \\
% 12011         &     1.20\% &       42.12 &     \bf{43.30} &       41.03 \\
% 29125         &     1.04\% &  \bf{56.50} &          54.10 &       52.32 \\
% 10060         &     1.00\% &       48.73 &     \bf{52.25} &       45.15 \\
% 69436         &     0.96\% &       85.18 &     \bf{88.32} &       83.30 \\
% 12002         &     0.91\% &       28.36 &     \bf{28.43} &       25.53 \\
% 59025         &     0.91\% &       69.00 &          67.73 &  \bf{73.82} \\
% 11042         &     0.89\% &       63.45 &     \bf{66.86} &       64.38 \\
% 47562         &     0.80\% &       76.25 &     \bf{77.67} &       70.74 \\
% 62323         &     0.79\% &       57.07 &     \bf{64.25} &       61.17 \\
% 64483         &     0.77\% &  \bf{67.32} &          66.74 &       54.27 \\
% 20610         &     0.75\% &       46.75 &     \bf{48.60} &       43.90 \\
% 43235         &     0.75\% &  \bf{38.77} &          35.45 &       31.43 \\
% 49083         &     0.63\% &       71.49 &     \bf{75.08} &       58.24 \\
% 51702         &     0.58\% &       20.30 &          22.96 &  \bf{24.74} \\
% \midrule
% \midrule
% Average &            &       60.40 &     \bf{61.26} &       58.02 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT codes\hancomment{Logistic Regression to be added later}}
% \label{tb:top20_svm}
% \end{table}



% \begin{table}[]
% \centering
% \begin{tabular}{llll}
% \toprule
% {} &       ELDAN & ELDAN+transfer &        ELDN \\
% \midrule
% 43239         &  \bf{86.21} &          84.93 &       84.59 \\
% 45380         &  \bf{75.14} &          74.02 &       72.68 \\
% 45385         &  \bf{72.33} &          70.31 &       71.33 \\
% 66984         &       92.87 &     \bf{93.00} &       92.15 \\
% 45378         &       65.45 &     \bf{67.57} &       62.67 \\
% 12001         &       44.74 &          43.62 &  \bf{46.96} \\
% 47562         &       76.25 &     \bf{77.67} &       70.74 \\
% 44970         &  \bf{70.63} &          69.63 &       63.97 \\
% 29125         &  \bf{56.50} &          54.10 &       52.32 \\
% 69436         &       85.18 &     \bf{88.32} &       83.30 \\
% 11042         &       63.45 &     \bf{66.86} &       64.38 \\
% 12011         &       42.12 &     \bf{43.30} &       41.03 \\
% 12002         &       28.36 &     \bf{28.43} &       25.53 \\
% 43235         &  \bf{38.77} &          35.45 &       31.43 \\
% 52332         &  \bf{47.38} &          44.63 &       36.90 \\
% 10060         &       48.73 &     \bf{52.25} &       45.15 \\
% 58558         &       58.88 &     \bf{60.27} &       52.12 \\
% 52356         &  \bf{63.61} &          58.48 &       47.79 \\
% 27447         &       52.20 &     \bf{59.35} &       47.72 \\
% 59025         &       69.00 &          67.73 &  \bf{73.82} \\
% \midrule
% \midrule
% Macro Average &       61.89 &     \bf{62.00} &       58.33 \\
% \bottomrule
% \end{tabular}
% \caption{Performance of 20 most frequent CPT code (without SVM)}
% \label{tb:top20}
% \end{table}









% \begin{enumerate}
%     \item Check with Guoli about the details of the experiment data for code assignment.
        
%         Need to make sure there is a reasonable story about this being a valid comparison (even if the datasets in the experimental conditions were only comparable, not identical, because of the need to compare against a highly tuned, production-level system).
        
%         Also need to check with Guoli about it being ok to report numbers from the production-level system.
        
%     \item Performance comparison:
%     \begin{enumerate}
%         \item Models:
%         \begin{enumerate}
%             \item ELDAN
%             \item ELDN (without attention, just averaging)
%             \item SVM OVA (3M current model, solution (1))
%         \end{enumerate}
        
%         \item ELDAN consistently outperforms ELDN with about 1.5 f1-score
%         \item Compared with SVM OVA, ELDAN outperform on common codes, but not as competitive when codes are rare (although in most cases, both models don\'t work well.)
%         \item Low resource codes: The effect of naive transfer learning (a consistent improvement of 1 f1-score, especially for rare codes) 
%     \end{enumerate}
    
%     \item Attention:
    
%     Experienced medical coder hand-labeled 400 encounters. 
% High f1 of document source assignment compared to human using ELDAN.
    
% \end{enumerate}


% \subsection{Evaluation Approach/Study Design} 

% Before jumping into the results: what exactly are you evaluating?
% Tell us (or remind us) about your study design and evaluation
% criteria.  

% \subsection{Results on Application A} 

% Give us some numbers about how well your awesomeness works, especially
% in comparison to some baselines.  You should provide a summary of the
% results in the text, as well as in tables (such as
% table~\ref{tab:example}) and figures (such as figure~\ref{fig:example}).  

% You may use subfigures/wrapfigures so that figures don't have to span
% the whole page or multiple figures are side by side.

% \begin{table}[htbp]
%   \centering 
%   \caption{These are our results.} 
%   \begin{tabular}{|l|l|}\hline
%     Us & Top Score \\ \hline
%     Baseline & Less Impressive Score \\ \hline 
%   \end{tabular}
%   \label{tab:example} 
% \end{table}

% \begin{figure}[htbp]
%   \centering 
%   \includegraphics[width=1.5in]{smile.jpeg} 
%   \caption{Feeling awesome.}
%   \label{fig:example} 
% \end{figure} 

% \subsection{Results on Application B} 

% Did more than one experiment type?  Sweet! 
